Spin transport properties in a topological insulator sandwiched between two-dimensional magnetic layers

Nontrivial band topology along with magnetism leads to different novel quantum phases. When time-reversal-symmetry is broken in three-dimensional topological insulators (TIs) by applying high enough magnetic field or proximity effect, different phases such as quantum Hall or quantum anomalous Hall(QAH) emerge and display interesting transport properties for spintronic applications. The QAH phase displays sidewall chiral edge states which leads to the QAH effect. In a finite slab, contribution of the surface states depends on both the cross-section and thickness of the system. Having a small cross-section and a thin thickness leads to direct coupling of the surfaces, on the other hand, a thicker slab results in a higher contribution of the non-trivial sidewall states which connect top and bottom surfaces. In this regard, we have considered a heterostructure consisting of a TI, namely Bi2Se3, which is sandwiched between two-dimensional magnetic monolayers of CrI3 to study its topological and transport properties. Combining DFT and tight-binding calculations along with non-equilibrium Green's function formalism, we show that a well-defined exchange gap appears in the band structure in which spin polarised edge states flow. We also study the width and finite-size effect on the transmission and topological properties of this magnetised TI nanoribbon.

==> notes.tex <==
\anna{General project notes and information are collected in this file.}

Testing Swedish letters, large ÅÄÖ and small åäö.

Cite an arbitrary paper \cite{Farhan2017,Carrera2015,Farhan2013}.
